Hierarchical Multimodal Pre-training for Visually Rich Webpage Understanding

The growing prevalence of visually rich documents, such as webpages and scanned/digital-born documents (images, PDFs, etc.), has led to increased interest in automatic document understanding and information extraction across academia and industry. Although various document modalities, including image, text, layout, and structure, facilitate human information retrieval, the interconnected nature of these modalities presents challenges for neural networks. In this paper, we introduce WebLM, a multimodal pre-training network designed to address the limitations of solely modeling text and structure modalities of HTML in webpages. Instead of processing document images as unified natural images, WebLM integrates the hierarchical structure of document images to enhance the understanding of markup-language-based documents. Additionally, we propose several pre-training tasks to model the interaction among text, structure, and image modalities effectively. Empirical results demonstrate that the pre-trained WebLM significantly surpasses previous state-of-the-art pre-trained models across several webpage understanding tasks. The pre-trained models and code are available at https://github.com/X-LANCE/weblm.

==> tabs/noise_level.tex <==
\begin{table}[t]
    \caption{Experimental results on WebSRC dev set while introducing different levels of visual noise in TIM.}
    \centering
    \begin{tabular}{p{0.3cm}<{\centering}@{}lccc}
         \toprule
         \multicolumn{2}{c}{Method} & EM$\uparrow$ & F1$\uparrow$ & POS$\uparrow$ \\
        \midrule

        %  \multicolumn{2}{c|}{$\text{TIE}_{\text{MarkupLM}}$} & 80.80 & 84.30 & 92.67 \\
         \multicolumn{2}{l}{$\text{WebLM}_{\text{BASE}}$+50\% visual noise} & 67.43 & 76.93 & 88.60 \\
         &  + 20\% visual noise & $\text{66.46}$ & $\text{75.60}$ & $\text{	87.45}$ \\
         & + 100\% visual noise & $\text{66.18}$ & $\text{75.33}$ & $\text{87.33}$\\
         & + 200\% visual noise & $\text{65.88}$ & $\text{74.55}$ & $\text{86.89}$\\
         \bottomrule
    \end{tabular}
    \label{tab:noise_level}
\end{table}

==> tabs/structural_visual_feature.tex <==
\begin{table}[t]
    \caption{Ablation study of visual structure on WebSRC dev set. }
    \centering
    \resizebox{\columnwidth}{!}{\begin{tabular}{p{0.3cm}<{\centering}@{-}lccc}
         \toprule
         \multicolumn{2}{c}{Method} & EM$\uparrow$ & F1$\uparrow$ & POS$\uparrow$ \\
        \midrule

        %  \multicolumn{2}{c|}{$\text{TIE}_{\text{MarkupLM}}$} & 80.80 & 84.30 & 92.67 \\
         \multicolumn{2}{l}{$\text{WebLM}_{\text{BASE}}$+Complete Visual Structure} & 67.43 & 76.93 & 88.60 \\
         &  $\text{25\%}$ Visual Structure & $\text{66.46}$ & $\text{76.60}$ & $\text{	88.45}$ \\
         & $\text{50\%}$ Visual Structure& $\text{66.18}$ & $\text{75.33}$ & $\text{88.33}$\\
         & $\text{75\%}$ Visual Structure & $\text{65.94}$ & $\text{74.02}$ & $\text{86.68}$ \\
         & $\text{100\%}$ Visual Structure & $\text{65.50}$ & $\text{73.88}$ & $\text{86.23}$ \\
         \bottomrule
    \end{tabular}}
    \label{tab:visual_ablation}
\end{table}

==> tabs/tag_table.tex <==
\begin{table}[h]
\caption{We categorize all tags into 12 classes {\footnotemark} and initialize tag embeddings using the vector representations of each tag's description.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Category}    & \textbf{Example} & \textbf{Tag Description}                \\ \midrule
Basic HTML           & <html>                       & Defines an HTML document                \\
Formatting           & <b>                          & Defines bold text                       \\
Forms and Input      & <button>                     & Defines a clickable button              \\
Styles and Semantics & <div>                        & Defines a section in a document         \\
Tables               & <th>                         & Defines a header cell in a table        \\
Lists                & <ul>                         & Defines an unordered list               \\
Images               & <img>                        & Defines an image                        \\
Audio/Video          & <audio>                      & Defines sound content                   \\
Links                & <a>                          & Defines a hyperlink                     \\
Frames               & <iframe>                     & Defines an inline frame                 \\
Meta Info            & <meta>                       & Defines metadata about HTML \\
Programming          & <script>                     & Defines a client-side script                                 \\ \bottomrule
\end{tabular}%
}
\label{tab:tag_list}
\end{table}

\footnotetext{https://www.w3schools.com/tags/ref\_byfunc.asp}
